On the Hierarchical Preconditioning of the Combined Field Integral Equation

This paper analyzes how hierarchical bases preconditioners constructed for the Electric Field Integral Equation (EFIE) can be effectively applied to the Combined Field Integral Equation (CFIE). For the case where no hierarchical solenoidal basis is available (e.g., on unstructured meshes), a new scheme is proposed: the CFIE is implicitly preconditioned on the solenoidal Helmholtz subspace by using a Helmholtz projector, while a hierarchical non-solenoidal basis is used for the non-solenoidal Helmholtz subspace. This results in a well-conditioned system. Numerical results corroborate the presented theory.

==> sacommands.tex <==
\newcommand{\bJ}{\operatorname{J}}
\newcommand{\bH}{\operatorname{H}}
\newcommand{\bN}{\operatorname{N}}
\newcommand{\ess}{\operatorname{ess}}
\newcommand{\e}{\mathrm{e}}
\newcommand{\jm}{\mathrm{j}}
\newcommand{\ep}{\varepsilon}
\newcommand{\sg}{\varsigma}
\newcommand{\mr}{\mathrm}
\newcommand{\ms}{\mathsf}
\newcommand{\mc}{\mathcal}
\newcommand{\wt}{\widetilde}

\newcommand{\bZ}{\operatorname{Z}}
\newcommand{\Span}{\operatorname{span}}
\newcommand{\ld}{\log_2}
\newcommand{\tr}{\mathrm{tr}}

\newcommand{\veg}[1]{\bm{#1}}     % geometrical / physical vectors
\newcommand{\vet}[1]{\bm{ \mathfrak{#1}}}    % I used it for physical vectors with time-dependency
\newcommand{\mat}[1]{\mathsfbfit{#1}} % n x n-dimensional matrix
\newcommand{\uv}[1]{\hat{\veg{#1}}} % unit vectors
\renewcommand{\vec}[1]{\mathsfbfit{#1}} %n-dimensional vector
\newcommand{\op}[1]{\mathcal{#1}} % operator that takes a scalar-valued function
\newcommand{\vecop}[1]{\bm{\mathcal{#1}}} % operator that takes a vector-valued function
\newcommand{\mel}[1]{\mathsfit{#1}}
\newcommand{\vel}[1]{\mathsfit{#1}}


%\DeclareMathOperator{\vcurl}{\stackrel{\longrightarrow}{curl}}
\DeclareMathOperator{\vcurl}{\mathbf{curl}}
\newcommand{\n}{\hat{\bm{n}}} 
\newcommand{\np}{\hat{\bm{n}}^\prime}  
\newcommand{\pn}{\partial_{\hat{\bm{n}}}} 
\newcommand{\pnp}{\partial_{\hat{\bm{n}}^\prime}}  
\newcommand{\pnnp}{\partial_{\hat{\bm{n}},\hat{\bm{n}}^\prime}}    
\newcommand{\hek}{\hat{\bm{e}}_k}

\newcommand\restr[2]{{% we make the whole thing an ordinary symbol
  \left.\kern-\nulldelimiterspace % automatically resize the bar with \right
  #1 % the function
  \vphantom{|} % pretend it's a little taller at normal size
  \right|_{#2} % this is the delimiter
  }}
  

\newcommand\rst[3]{{% we make the whole thing an ordinary symbol
  \left.\kern-\nulldelimiterspace % automatically resize the bar with \right
  #1 % the function
  \vphantom{|} % pretend it's a little taller at normal size
  \right|_{#2}^{#3} % this is the delimiter
  }}
    
%\newenvironment{rcases}{%
%  \left.\renewcommand*\lbrace.%
%  \begin{cases}}%
%{\end{cases}\right\rbrace} 


\newcommand{\ZA}{\mat{Z}_\ms{A}}    
\newcommand{\ZPhi}{\mat{Z}_\Phiup}    

\newcommand{\matL}{\mat{\Lambda}}   
\newcommand{\matS}{\mat{\Sigma}}

\newcommand{\matLT}{\widetilde{\mat{\Lambda}}}   
\newcommand{\matST}{\widetilde{\mat{\Sigma}}}

\newcommand{\matLr}{\mat{\Lambda}_\ms{r}}
\newcommand{\matSr}{\mat{\Sigma}_\ms{r}}

\newcommand{\Pl}{\mat P_{\upLambda}}
\newcommand{\Ps}{\mat P_{\upSigma}}
\newcommand{\Ph}{\mat P_\mr{H}}
\newcommand{\Plh}{\mat P_\ms{\Lambda H}}
\newcommand{\T}{\ms{T}}
\newcommand{\Ht}{\ms{H}}
\newcommand{\matI}{\mat I}
\newcommand{\matO}{\mat 0}
\newcommand{\vecO}{\bm{\mathsf{0}}}

\newcommand{\iL}{\vec i_\ms{\Lambda}}
\newcommand{\iS}{\vec i_\ms{\Sigma}}
\newcommand{\iH}{\vec i_\ms{H}}

\newcommand{\matHL}{\mat L}
\newcommand{\matHS}{\mat S}
\newcommand{\matDL}{\mat D_\ms{L}}
\newcommand{\matDS}{\mat D_\ms{S}}

\newcommand{\LapLinv}{\(\matL^\T \matL\)^+}
\newcommand{\LapLGLinv}{\(\matL^\T \mat G \matL\)^+}
\newcommand{\LapSinv}{\(\matS^\T \matS\)^+}
\newcommand{\LapSGSinv}{\(\matS^\T \mat G^\ms{BC} \matS\)^+}

\newcommand{\Gpyr}{\mat G_{\lambda\lambda}}
\newcommand{\GpyrInv}{\mat G_{\lambda\lambda}^{-1}}
\newcommand{\Gbcpatchpyr}{\mat G_{\ms{p^{BC}}\lambda}}
\newcommand{\Gbcpatch}{\mat G_{\ms{p^{BC}p^{BC}}}}
\newcommand{\HTransfL}{\mat H_\ms{TransfL}}
\newcommand{\HTransfS}{\mat H_\ms{TransfS}}

\newcommand{\LapL}{\matL^\T \matL}
\newcommand{\LapS}{\matS^\T \matS}
\newcommand{\LapLLinv}{\(\matL \matL^\T\)^+}
\newcommand{\LapSSinv}{\(\matS \matS^\T\)^+}

\newcommand{\LapLL}{\matL \matL^\T}
\newcommand{\LapSS}{\matS \matS^\T}

\newcommand{\LapLr}{\matLr^\T \matLr}
\newcommand{\LapSr}{\matSr^\T \matSr}

\newcommand{\LapLsinv}{\(\matL^\T \matL\)^{-1/2}}
\newcommand{\LapSsinv}{\(\matS^\T \matS\)^{-1/2}}


\newcommand{\bt}{\bm t}
\DeclareMathOperator{\ran}{ran}

%geändertes Label-Makro, damit man auch mit hyperref auf Labels verweisen kann!
\newcommand{\jlabel}[1]{\hypertarget{#1}{}\label{#1}}



% Befehle für Index-Erstellung
\newcommand{\itindex}[1]{{{\index{#1}}#1}} % Index-Eintrag im Fließtext. Es wird der Eintrag selbe auch ausgegeben.
\newcommand{\itindexbf}[1]{{\textbf{{\index{#1}}#1}}}
\newcommand{\itindexit}[1]{{\textit{{\index{#1}}#1}}}


%zur Fehlerbehebung bei Verwendung mit TeXnicCenter 4 beta
\newcommand{\p}{\\[3mm]}
\newcommand{\script}{\scriptsize}


% Vektoren
%\renewcommand{\arraystretch}{1.4}

\newcommand{\twovector}[2]{\begin{pmatrix} #1 \\ #2 \end{pmatrix}} % Vektor mit zwei zwei Einträgen
\newcommand{\smalltwovector}[2]{\left(\begin{smallmatrix} #1 \\ #2 \end{smallmatrix}\right)} 
\newcommand{\jvector}[3]{\begin{array}{c} #1 \\ #2 \\ #3 \end{array}} % Vektor mit drei Einträgen
\newcommand{\threevector}[3]{\begin{pmatrix} #1 \\ #2 \\ #3 \end{pmatrix}} % Vektor mit drei Einträgen
\newcommand{\smallthreevector}[3]{\left(\begin{smallmatrix} #1 \\ #2 \\ #3 \end{smallmatrix}\right)} % kleiner Vektor mit drei Einträgen
\newcommand{\fourvector}[4]{\begin{pmatrix} #1 \\ #2 \\ #3 \\ #4 \end{pmatrix}} % Vektor mit vier Einträgen
\newcommand{\smallfourvector}[4]{\left(\begin{smallmatrix} #1 \\ #2 \\ #3 \\ #4\end{smallmatrix}\right)}% kleiner Vektor mit vier Einträgen
 \newcommand{\vecn}[2]{\begin{pmatrix} #1 \\\vdots\\ #2 \end{pmatrix}} % Vektor der Form (x_1 ... x_n)
\newcommand{\vecxnsmall}{\left(\begin{smallmatrix} x_1 \\ \vdots \\ x_n \end{smallmatrix}\right)}
\newcommand{\vecynsmall}{\left(\begin{smallmatrix} y_1 \\ \vdots \\ y_n \end{smallmatrix}\right)}
\newcommand{\vecxntsmall}{\left(x_1,\ldots,x_n\right)}
\newcommand{\vecyntsmall}{\left(y_1,\ldots,y_n\right)}

% Matritzen
\newcommand{\fourmatrix}[4]{\begin{pmatrix} #1 & #2 \\ #3 & #4 \end{pmatrix}} % 2x2-Matrix

% spezielle Matritzen
\newcommand{\matAmnsmall}{\left(\begin{smallmatrix} a_{11} & \ldots & a_{1n}\\ \vdots & \ddots & \vdots \\  a_{n1} & \ldots & a_{nn}\end{smallmatrix}\right)} % kleine nxn-Matrix mit Einträgen a_ij
\newcommand{\matBmnsmall}{\left(\begin{smallmatrix} b_{11} & \ldots & b_{1n}\\ \vdots & \ddots & \vdots \\  b_{n1} & \ldots & b_{nn}\end{smallmatrix}\right)} % kleine nxn-Matrix mit Einträgen b_ij
\newcommand{\matCmnsmall}{\left(\begin{smallmatrix} c_{11} & \ldots & c_{1n}\\ \vdots & \ddots & \vdots \\  c_{n1} & \ldots & c_{nn}\end{smallmatrix}\right)}% kleine nxn-Matrix mit Einträgen c_ij
\newcommand{\matTmnsmall}{\left(\begin{smallmatrix} t_{11} & \ldots & t_{1n}\\ \vdots & \ddots & \vdots \\  t_{n1} & \ldots & t_{nn}\end{smallmatrix}\right)}% kleine nxn-Matrix mit Einträgen t_ij
\newcommand{\matAmn}{\left(\begin{array}{cccc}a_{11} & a_{12} & \ldots & a_{1n}\\a_{21} & a_{22} & \ldots & a_{2n}\\\vdots &\vdots &\ddots & \vdots\\a_{m1} & a_{m2} & \ldots & a_{mn}\\\end{array}\right)} % mxn-Matrix mit Einträgen a_ij
\newcommand{\matAnn}{\left(\begin{array}{cccc}a_{11} & a_{12} & \ldots & a_{1n}\\a_{21} & a_{22} & \ldots & a_{2n}\\\vdots & & & \vdots\\a_{n1} & a_{n2} & \ldots & a_{nn}\\\end{array}\right)} % nxn-Matrix mit Einträgen a_ij
\newcommand{\matEnBig}{\left(\begin{array}{cccc}1 & 0 & \ldots & 0\\0 & 1 & \ddots & \vdots\\\vdots & \ddots & \ddots& 0\\0 & \ldots & 0 & 1\\\end{array}\right)} % große nxn-Einheitsmatrix
\newcommand{\matEn}{\left(\begin{array}{cc}1 & \mathbf{0} \\ \mathbf{0} & 1\end{array}\right)} % Einheitsmatrix
\newcommand{\matDiag}[2]{\begin{pmatrix}#1 &  & \mathbf{0}\\  & \ddots & \\ \mathbf{0} &  & #2\end{pmatrix}} % Diagonalmatrix mit Einträgen x_1..x_2 auf der Diagonalen
\newcommand{\matThreeDiag}[3]{\begin{pmatrix}#1 & 0 & 0\\ 0 & #2 & 0\\ 0 & 0 & #3\end{pmatrix}} % 3x3-Diagonalmatrix
\newcommand{\matTriangle}[2]{\begin{pmatrix}#1 & \cdots & \\  & \ddots & \vdots\\ \mathbf{0}&  & #2\end{pmatrix}} % rechte obere Dreiecksamtrix

%Determinanten
\newcommand{\fourdet}[4]{\begin{vmatrix} #1 & #2 \\ #3 & #4 \end{vmatrix}}

% Real- und Imaginärteil-Operatoren
\renewcommand{\Re}{\mathrm{Re}\;}
\renewcommand{\Im}{\mathrm{Im}\;}


% Darstellung von Einheiten
%\newcommand{\unit}[1]{\:\mathrm{#1}}
%\newcommand{\unitf}[2]{\:\mathrm{\frac{#1}{#2}}}


\newcommand{\const}{{\text{const}}}


% Differentialbrüche
\newcommand{\ntfrac}[2]{\frac{\nt{#1}}{\nt{#2}}}  % partielles Differential
\newcommand{\pfrac}[2]{\frac{\uppartial #1}{\uppartial #2}}  % partielles Differential
\newcommand{\fracpd}[2]{\frac{\uppartial #1}{\uppartial #2}} % partielles Differential
\newcommand{\fracppd}[2]{\frac{\uppartial^2 #1}{\uppartial #2^2}}  % zweite partielle 
\newcommand{\fracd}[2]{\frac{\mathrm{d} #1}{\mathrm{d} #2}} % partielles Differential
\newcommand{\fracdd}[2]{\frac{\mathrm{d}^2 #1}{\mathrm{d} #2^2}}  % zweite partielle 


\newcommand{\dd}{\mathrm{d}}  
\newcommand{\ii}{\mathrm{i}}  

% Blackboard-Font: Bezeichnungen für Mengen
\newcommand{\bbone}{\mathds{1}}  % mathds benötigt das Package "dsfont"
\newcommand{\C}{\mathbb{C}}
\newcommand{\K}{\mathbb{K}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\bP}{\mathbb{P}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Z}{\mathbb{Z}}


% spezielle Mengen R^n etc.
\newcommand{\Knn}{\mathbb{K}^{n\times n}}
\newcommand{\Kmn}{\mathbb{K}^{m\times n}}
\newcommand{\Rnnn}{\mathbb{R}^{n\times n}}
\newcommand{\Rmn}{\mathbb{R}^{m\times n}}
\newcommand{\Rmm}{\mathbb{R}^{m\times m}}
\newcommand{\Kn}{\mathbb{K}^n}
\newcommand{\Rnn}{\mathbb{R}^n}
\newcommand{\Rthree}{\mathbb{R}^3}
\newcommand{\Km}{\mathbb{K}^m}
\newcommand{\Rm}{\mathbb{R}^m}
\newcommand{\HM}{\mathcal{H}(M)}
\newcommand{\KX}{K\left[X\right]} %Menge der Polynome über X (???)
\newcommand{\jset}[2]{\bigl\{ #1 \bigl| #2 \bigr.\bigr\}} % Menge aller Elemente #1 mit Eigenschaft #2
\newcommand{\mCab}{{\cC}\left[a,b\right]} % C[a,b]
\newcommand{\Cab}{{$\mCab$}} % Cab außerhalb Mathe-Modus



% Größen mit Hut
\newcommand{\hx}{\hat{x}}
\newcommand{\hlambda}{\hat{\lambda}}
\newcommand{\hy}{\hat{y}}

% häufige Grenzübergänge
\newcommand{\limninfty}{\lim\limits_{n\rightarrow\infty}} % lim n -> infty
\newcommand{\limkinfty}{\lim\limits_{k\rightarrow\infty}} % lim k -> infty
\newcommand{\liminfninfty}{\liminf\limits_{n\rightarrow\infty}} % liminf n-> infty
\newcommand{\liminfkinfty}{\liminf\limits_{k\rightarrow\infty}} % liminf k-> infty
\newcommand{\limsupninfty}{\limsup\limits_{n\rightarrow\infty}} % limsup n-> infty
\newcommand{\limsupkinfty}{\limsup\limits_{k\rightarrow\infty}} % limsup k-> infty
\newcommand{\supnN}{\sup\limits_{n\in\N}} % sup n in N
\newcommand{\infnN}{\sup\limits_{n\in\N}} % inf n in N
\newcommand{\ninfty}{n\rightarrow\infty} % n -> infty
\newcommand{\kinfty}{k\rightarrow\infty} % k -> infty
\newcommand{\epsilonzero}{\epsilon\rightarrow0} % epsilon -> 0
\newcommand{\epsilonnull}{\epsilon\rightarrow0} % epsilon -> 0
\newcommand{\hzero}{h\rightarrow0} % h -> 0
\newcommand{\hnull}{h\rightarrow0} % h -> 0

% häufige Summationen
\newcommand{\sumknullinfty}{\sum\limits_{k=0}^\infty}
\newcommand{\sumnnullinfty}{\sum\limits_{n=0}^\infty}
\newcommand{\sumkzeroinfty}{\sum\limits_{k=0}^\infty}
\newcommand{\sumnzeroinfty}{\sum\limits_{n=0}^\infty}
\newcommand{\sumkoneinfty}{\sum\limits_{k=1}^\infty}
\newcommand{\sumkonen}{\sum\limits_{k=1}^n}
\newcommand{\sumkonem}{\sum\limits_{k=1}^m}
\newcommand{\sumionen}{\sum\limits_{i=1}^n}
\newcommand{\sumjonen}{\sum\limits_{j=1}^n}
\newcommand{\sumionem}{\sum\limits_{i=1}^m}
\newcommand{\sumnoneinfty}{\sum\limits_{n=1}^\infty}

% diverse Operatoren/Funktionen etc.

% lineare Algebra (Normen etc.)
\newcommand{\sabs}[1]{{|#1|}} % Absolut-Betrag

\newcommand{\bigabs}[1]{\bigl|#1\bigr|} % Absolut-Betrag, groß
\newcommand{\absa}[1]{\left|#1\right|_a}
\newcommand{\absi}[1]{\left|#1\right|_i}

\newcommand{\norm}[1]{\left\Vert #1 \right\Vert} % Norm
\newcommand{\nt}[1]{\left\Vert #1 \right\Vert_2} % Norm
\newcommand{\nf}[1]{\left\Vert #1 \right\Vert_\mr{F}} % Norm
\newcommand{\normmax}[1]{\left\|#1\right\|_{\infty}} % infty-Norm
\newcommand{\normltwo}[1]{\left\|#1\right\|_{L^2}} % L2-Norm
\newcommand{\transp}[1]{{#1}^t} % Transposition
\newcommand{\pair}[2]{\langle #1, #2 \rangle}
\newcommand{\Ltp}[2]{\(#1,#2\)_{L^2}}

% spezielle Befehle: Physik
\newcommand{\lorentz}{\textsc{Lorentz}}
\newcommand{\einstein}{\textsc{Einstein}}
\newcommand{\smallmetric}{\left(\begin{smallmatrix}1 & & &\mathbf{0}\\ & -1 & &\\ & & -1 &\\\mathbf{0} & & &-1\\\end{smallmatrix}\right)} % Metrik der spec. Rel.
\newcommand{\poisson}[2]{\left\{{#1},{#2}\right\}}

%Quantenmechanische Bra-Ket-Notation
\newcommand{\bra}[1]{\langle{#1}|}
\newcommand{\ket}[1]{|{#1}\rangle}
\newcommand{\braOPket}[3]{\langle #1|\hat{#2}| #3\rangle}
\newcommand{\braOPvket}[3]{\langle #1|\hat{\vec{#2}}| #3\rangle}
\newcommand{\braopket}[3]{\langle #1| #2 | #3\rangle}
\newcommand{\braket}[2]{\langle #1 | #2 \rangle}
\newcommand{\ketbra}[2]{\ket{#1}\bra{#2}}
\newcommand{\qmskalar}[2]{\langle #1, #2 \rangle}
\newcommand{\OP}[1]{\hat{\mathrm{#1}}}
\newcommand{\OPv}[1]{\hat{\vec{\mathrm{#1}}}}
\newcommand{\obs}[1]{\mathcal{#1}}
\newcommand{\obsv}[1]{\vec{\mathcal{#1}}}
\newcommand{\commutator}[2]{[#1, #2]}
\newcommand{\commutatorOP}[2]{[\hat{#1}, \hat{#2}]}
\newcommand{\commutatorOPv}[2]{[\hat{\vec{#1}}, \hat{#2}]}
\newcommand{\acommutator}[2]{\{#1, #2\}}
\newcommand{\acommutatorOP}[2]{\{\hat{#1}, \hat{#2}\}}
\newcommand{\acommutatorOPv}[2]{\{\hat{\vec{#1}}, \hat{#2}\}}
\newcommand{\smean}[1]{\bigl\langle #1\bigr\rangle}
\newcommand{\mean}[1]{\left\langle #1\right\rangle}
\newcommand{\meanOP}[1]{\langle\hat{#1}\rangle}
\newcommand{\meanOPv}[1]{\langle\hat{\vec{#1}}\rangle}
\newcommand{\prob}[1]{\bP\left({#1}\right)}
\newcommand{\tp}{\otimes}

\newcommand{\ketupsdown}{\ket{\uparrow/\downarrow}}
\newcommand{\braupsdown}{\bra{\uparrow/\downarrow}}

\newcommand{\ketupup}{\ket{\uparrow\uparrow}}
\newcommand{\braupup}{\bra{\uparrow\uparrow}}
\newcommand{\ketupdown}{\ket{\uparrow\downarrow}}
\newcommand{\braupdown}{\bra{\uparrow\downarrow}}
\newcommand{\ketdownup}{\ket{\downarrow\uparrow}}
\newcommand{\bradownup}{\bra{\downarrow\uparrow}}
\newcommand{\ketdowndown}{\ket{\downarrow\downarrow}}
\newcommand{\bradowndown}{\bra{\downarrow\downarrow}}
\newcommand{\ketup}{\ket{\uparrow}}
\newcommand{\braup}{\bra{\uparrow}}
\newcommand{\ketdown}{\ket{\downarrow}}
\newcommand{\bradown}{\bra{\downarrow}}
\newcommand{\ketnlm}{\ket{nlm}}
\newcommand{\branlm}{\bra{nlm}}
\newcommand{\ketp}{\ket{p}}
\newcommand{\ketq}{\ket{q}}
\newcommand{\ketn}{\ket{n}}
\newcommand{\keta}{\ket{a}}
\newcommand{\braa}{\bra{a}}
\newcommand{\ketb}{\ket{b}}
\newcommand{\brab}{\bra{b}}
\newcommand{\ketr}{\ket{r}}
\newcommand{\brar}{\bra{r}}
\newcommand{\ketpsi}{\ket{\psi}}
\newcommand{\ketphi}{\ket{\phi}}
\newcommand{\brap}{\bra{p}}
\newcommand{\braq}{\bra{q}}
\newcommand{\bran}{\bra{n}}
\newcommand{\brapsi}{\bra{\psi}}
\newcommand{\braphi}{\bra{\phi}}
\newcommand{\OPA}{\OP{A}}
\newcommand{\OPvA}{\OPv{A}}
\newcommand{\OPa}{\OP{a}}
\newcommand{\OPadagger}{{\OP{a}^\dagger}}
\newcommand{\OPad}{\OPadagger}
\newcommand{\OPB}{\OP{B}}
\newcommand{\OPC}{\OP{C}}
\newcommand{\OPD}{\OP{D}}
\newcommand{\OPE}{\OP{E}}
\newcommand{\OPF}{\OP{F}}
\newcommand{\OPG}{\OP{G}}
\newcommand{\OPH}{\OP{H}}
\newcommand{\OPI}{\OP{I}}
\newcommand{\OPJ}{\OP{J}}
\newcommand{\OPJs}{\OP{J}^2}
\newcommand{\OPJx}{\OP{J}_x}
\newcommand{\OPJpm}{\OP{J}_{\pm}}
\newcommand{\OPJmp}{\OP{J}_{\mp}}
\newcommand{\OPJp}{\OP{J}_{+}}
\newcommand{\OPJm}{\OP{J}_{-}}
\newcommand{\OPJy}{\OP{J}_y}
\newcommand{\OPJz}{\OP{J}_z}
\newcommand{\OPJv}{\OPv{J}}
\newcommand{\OPJvs}{\OPv{J}^2}
\newcommand{\OPvJ}{\OPJv}
\newcommand{\OPK}{\OP{K}}
\newcommand{\OPk}{\OP{k}}
\newcommand{\OPL}{\OP{L}}
\newcommand{\OPLs}{\OP{L}^2}
\newcommand{\OPLp}{\OP{L}_{+}}
\newcommand{\OPLpm}{\OP{L}_{\pm}}
\newcommand{\OPLmp}{\OP{L}_{\mp}}
\newcommand{\OPLm}{\OP{L}_{-}}
\newcommand{\OPLx}{\OP{L}_x}
\newcommand{\OPLy}{\OP{L}_y}
\newcommand{\OPLz}{\OP{L}_z}
\newcommand{\OPLv}{\OPv{L}}
\newcommand{\OPvL}{\OPLv}
\newcommand{\OPLvs}{\OPv{L}^2}
\newcommand{\OPM}{\OP{M}}
\newcommand{\OPN}{\OP{N}}
\newcommand{\OPn}{\OP{n}}
\newcommand{\OPO}{\OP{O}}
\newcommand{\OPP}{\OP{P}}
\newcommand{\OPvP}{\OPv{P}}
\newcommand{\OPQ}{\OP{Q}}
\newcommand{\OPvQ}{\OPv{Q}}
\newcommand{\OPp}{\OP{p}}
\newcommand{\OPq}{\OP{q}}
\newcommand{\OPR}{\OP{R}}
\newcommand{\OPr}{\OP{r}}
\newcommand{\OPvR}{\OPv{R}}
\newcommand{\OPS}{\OP{S}}
\newcommand{\OPSs}{\OP{S}^2}
\newcommand{\OPSp}{\OP{S}_{+}}
\newcommand{\OPSpm}{\OP{S}_{\pm}}
\newcommand{\OPSmp}{\OP{S}_{\mp}}
\newcommand{\OPSm}{\OP{S}_{-}}
\newcommand{\OPSx}{\OP{S}_x}
\newcommand{\OPSy}{\OP{S}_y}
\newcommand{\OPSz}{\OP{S}_z}
\newcommand{\OPSv}{\OPv{S}}
\newcommand{\OPvS}{\OPSv}
\newcommand{\OPSvs}{\OPv{S}^2}

\newcommand{\OPT}{\OP{T}}
\newcommand{\OPU}{\OP{U}}
\newcommand{\OPV}{\OP{V}}
\newcommand{\OPW}{\OP{W}}
\newcommand{\OPX}{\OP{X}}
\newcommand{\OPvX}{\OPv{X}}
\newcommand{\OPY}{\OP{Y}}
\newcommand{\OPZ}{\OP{Z}}
\newcommand{\OPx}{\OP{x}}
\newcommand{\OPy}{\OP{y}}
\newcommand{\OPz}{\OP{z}}
\newcommand{\OPPi}{\OP{\Pi}}




% sonstige Befehle
\newcommand{\txt}[1]{{\text{#1}}} % Text in Mathe-Umgebung (aufrecht gesetzt)
\newcommand{\txttt}[1]{{\text{\texttt{#1}}}}

%\newcommand{\jgraphics}[2]{\parbox{#1}{\begin{latexonly}\includegraphics{#2.pdf}\end{latexonly}\html{\includegraphics{../epsfig/#2.eps}}}}
\newcommand{\jgraphics}[2]{\parbox{#1}{\includegraphics{#2.pdf}}}


% diverse Mathe-Operatoren
\DeclareMathOperator{\dalembert}{\square}
\DeclareMathOperator{\ee}{e}
\DeclareMathOperator{\arcsinh}{arcsinh}
\DeclareMathOperator{\arccosh}{arccosh}
\DeclareMathOperator{\arctanh}{arctanh}
\DeclareMathOperator{\sinc}{sinc}
\DeclareMathOperator{\tanc}{tanc}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\dist}{dist}
\DeclareMathOperator{\cond}{cond}
\DeclareMathOperator{\Div}{div}
\DeclareMathOperator{\rot}{rot}
\DeclareMathOperator{\curl}{curl}
\DeclareMathOperator{\Var}{Var}
\DeclareMathOperator{\Lin}{Lin}
\DeclareMathOperator{\Rang}{Rang}
\DeclareMathOperator{\Ker}{Ker}
\DeclareMathOperator{\Null}{null}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\Img}{Im}
\DeclareMathOperator{\Hom}{Hom}
\DeclareMathOperator{\id}{id}
\DeclareMathOperator{\End}{End}
\DeclareMathOperator{\GL}{GL}
\DeclareMathOperator{\SL}{SL}
\DeclareMathOperator{\Spur}{Spur}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\grad}{grad}
\DeclareMathOperator{\Eig}{Eig}
\DeclareMathOperator{\supp}{supp}



% Fourier-Trafos
\newcommand{\FT}{\cF}
\newcommand{\FTa}[1]{\cF\left[#1\right]}
\newcommand{\FTi}{\cF^{-1}}
\newcommand{\FTia}[1]{\cF^{-1}\left[#1\right]}


%% Booktabs

\newcolumntype {n}{c}
\newcolumntype {N}{>{\small}c}
\newcolumntype {L}{>{\small}l}
\newcolumntype {F}{>{\footnotesize}c}
\newcolumntype {v}[1]{>{\raggedright \hspace {0pt}} p {#1}}
\newcolumntype {V}[1]{>{\small \raggedright \hspace {0pt}} p {#1}}
\newcolumntype{d}[1]{>{\DC@{.}{.}{#1}}c<{\DC@end}}

\newcommand{\armultirow}[3]{%
  \multicolumn{#1}{#2}{%
    \begin{picture}(0,0)%
      \put(0,0){%
        \begin{tabular}[t]{@{}#2@{}}%
          #3%
        \end{tabular}%
      }%
    \end{picture}%
  }%
}%
% array.sty, rotating.sty
\newcolumntype{R}[1]{%
  >{\begin{turn}{90}\begin{minipage}{#1}\small\raggedright\hspace{0pt}}l%
  <{\end{minipage}\end{turn}}%
}



